Lotus-2: Advancing Geometric Dense Prediction with Powerful Image Generative Model

Recovering pixel-wise geometric properties from a single image is fundamentally ill-posed due to appearance ambiguity and non-injective mappings between 2D observations and 3D structures. While discriminative regression models achieve strong performance through large-scale supervision, their success is bounded by the scale, quality, and diversity of available data, as well as by limited physical reasoning. Recent diffusion models exhibit powerful world priors that encode geometry and semantics learned from massive image-text data, yet directly reusing their stochastic generative formulation is suboptimal for deterministic geometric inference: the former is optimized for diverse and high-fidelity image generation, whereas the latter requires stable and accurate predictions. In this work, we propose Lotus-2, a two-stage deterministic framework for stable, accurate and fine-grained geometric dense prediction, aiming to provide an optimal adaptation protocol to fully exploit the pre-trained generative priors. Specifically, in the first stage, the core predictor employs a single-step deterministic formulation with a clean-data objective and a lightweight local continuity module (LCM) to generate globally coherent structures without grid artifacts. In the second stage, the detail sharpener performs a constrained multi-step rectified-flow refinement within the manifold defined by the core predictor, enhancing fine-grained geometry through noise-free deterministic flow matching. Using only 59K training samples, less than 1% of existing large-scale datasets, Lotus-2 establishes new state-of-the-art results in monocular depth estimation and highly competitive surface normal prediction. These results demonstrate that diffusion models can serve as deterministic world priors, enabling high-quality geometric reasoning beyond traditional discriminative and generative paradigms.

==> sec/biography.tex <==
\section{Biography Section}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/authors/hj.jpg}}]{Jing He} is a Doctor of Philosophy student at AI Thrust of Hong Kong University of Science and Technology (Guangzhou). Her research interest lies in visual generative models and 3D vision. Prior to that, she received her Master's degree at the Information School of Xiamen University.   
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/authors/lhd.jpg}}]{Haodong Li} is a Doctor of Philosophy student at the Department of Computer Science \& Engineering, University of California San Diego, working with Professor Manmohan Chandraker. Prior to this, he got his Master of Philosophy degree at the AI Thrust of the Hong Kong University of Science and Technology (Guangzhou), working with Professor Ying-Cong Chen. He got his Bachelor of Engineering degree from Zhejiang University.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/authors/smz.JPG}}]{Mingzhi Sheng} Mingzhi Sheng received the bachelor’s degree from South China University of Technology in 2024. She is currently pursuing the Master of Philosophy degree in the AI Thrust at The Hong Kong University of Science and Technology (Guangzhou). Her research interests include generative AI for geometric perception, video generation and video editing. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/authors/cyc.jpg}}]{Ying-Cong Chen}
 is an Assistant Professor at AI Thrust of Hong Kong University of Science and Technology (Guangzhou), and also jointly appointed by the department of Computer Science \& Engineering. Prior to that, he was a Postdoctoral Associate at Computer Science \& Artificial Intelligence Lab of Massachusetts Institute of Technology. He has been dedicated to research in computer vision, particularly in visual generative models. His works have been published in top conferences and journals like TPAMI, CVPR, ICCV, ECCV, etc. His research achievements include being selected for ESI Highly Cited Papers, ICCV Best Paper Nomination, and winning the first prize in the Natural Science Award of the China Society for Image and Graphics. 
\end{IEEEbiography}


% If you have an EPS/PDF photo (graphicx package needed), extra braces are
%  needed around the contents of the optional argument to biography to prevent
%  the LaTeX parser from getting confused when it sees the complicated
%  $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
%  your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
%  simpler here.)
 
% \vspace{11pt}

% \bf{If you include a photo:}\vspace{-33pt}
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
% Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
% Use the author name as the 3rd argument followed by the biography text.
% \end{IEEEbiography}

% \vspace{11pt}

% \bf{If you will not include a photo:}\vspace{-33pt}
% \begin{IEEEbiographynophoto}{John Doe}
% Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
% \end{IEEEbiographynophoto}

